Adaptive Channel Recommendation For Opportunistic Spectrum Access

We propose a dynamic spectrum access scheme where secondary users recommend "good" channels to each other and access accordingly. We formulate the problem as an average reward based Markov decision process. We show the existence of the optimal stationary spectrum access policy, and explore its structure properties in two asymptotic cases. Since the action space of the Markov decision process is continuous, it is difficult to find the optimal policy by simply discretizing the action space and use the policy iteration, value iteration, or Q-learning methods. Instead, we propose a new algorithm based on the Model Reference Adaptive Search method, and prove its convergence to the optimal policy. Numerical results show that the proposed algorithms achieve up to 18% and 100% performance improvement than the static channel recommendation scheme in homogeneous and heterogeneous channel environments, respectively, and is more robust to channel dynamics.

==> Motivation.tex <==
%!TEX root = main.tex
%SourceDoc main.tex

\section{\label{sec:Motivation-Adaptive}Motivations For Adaptive Channel Recommendation}
The static channel recommendation mechanism is simple to implement due to a fixed value of $P_{rec}$. However, it may lead to significant congestions when the number of recommended channels is small. In the extreme case when only $R=1$ channel is recommended, calculation (\ref{eq:SCR-1}) suggests that every user will access that channel with a probability $P_{rec}$. When the number of users $N$ is large, the expected number of users accessing this channel $NP_{rec}$ will be high. Thus heavy congestion happens and each secondary user will get a low expected throughput.

A better way is to adaptively change the value of $P_{rec}$ based on the number of recommended channels. This is the key idea of our proposed algorithm.
To illustrate the advantage of adaptive algorithms, let us first consider a simple heuristic  adaptive algorithm. In this algorithm, we choose the branching probability such that the expected number of secondary users choosing a single recommended channel is one. To achieve this, we need to set $P_{rec}$ as in Lemma 2.
\begin{lem}\label{lemma12s}
If we choose the branching probability $P_{rec}=\frac{R}{N}$, then the expected number of secondary users choosing
any one of the $R$ recommended channels is one.
\end{lem}

Please refer to the Appendix for the detailed proof of Lemma \ref{lemma12s}.


Without going through detailed analysis, it is straightforward to show the benefit for such adaptive approach through simple numerical examples. Let us consider a network with $M=10$ channels and $N=5$ secondary users. For each channel $m$, the initial channel state probability vector is $\boldsymbol{p}_{m}(0)=(0,1)$
and the transition matrix is \[
\Gamma=\left[\begin{array}{cc}
1-0.01\epsilon & 0.01\epsilon\\
0.01\epsilon & 1-0.01\epsilon\end{array}\right],\]
where $\epsilon$ is called the dynamic factor. A larger value of $\epsilon$ implies that the channels are more dynamic over time.
We are interested in the time average system throughput
%
\[U=\frac{\sum_{t=1}^{T}\sum_{n=1}^{N}u_{n}(t)}{T},\]
%
where $u_{n}(t)$ is the throughput of user $n$ at time slot $t$. In the simulation, we set the total number of time slots $T=2000$.

We implement the following three channel access schemes:
\begin{itemize}
\item Random access scheme: each secondary user selects a channel randomly.
\item Static channel recommendation scheme as in \cite{key-2} with the \emph{optimal} constant branching
probability $P_{rec}=0.7$.
\item Heuristic adaptive channel recommendation scheme with the variable branching probability
$P_{rec}=\frac{R}{N}$.
\end{itemize}

Figure \ref{fig:Comparison-of-three} shows that the heuristic adaptive channel recommendation scheme outperforms the static channel recommendation scheme, which in turn outperforms the
random access scheme. Moreover, the heuristic adaptive scheme is more robust to the dynamic channel environment, as it decreases slower than the static scheme when $\epsilon$ increases.

%
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{Recommendation_System_Comparisons.eps}
\end{center}
\caption{\label{fig:Comparison-of-three}Comparison of three channel access
schemes}

\end{figure}


We can imagine that an optimal adaptive scheme (by setting the right $P_{rec}(t)$ over time) can further increase the network performance. However, computing the optimal branching probability in closed-form is very difficult. In the rest of the paper, we will focus on characterizing the structures of the optimal spectrum access strategy and designing an efficient algorithm to achieve the optimum.

